Policy Gradient in Partially Observable Environments: Approximation and Convergence

Policy gradient is a generic and flexible reinforcement learning approach that generally enjoys simplicity in analysis, implementation, and deployment. In the last few decades, this approach has been extensively advanced for fully observable environments. In this paper, we generalize a variety of these advances to partially observable settings, and similar to the fully observable case, we keep our focus on the class of Markovian policies. We propose a series of technical tools, including a novel notion of advantage function, to develop policy gradient algorithms and study their convergence properties in such environments. Deploying these tools, we generalize a variety of existing theoretical guarantees, such as policy gradient and convergence theorems, to partially observable domains, those which also could be carried to more settings of interest. This study also sheds light on the understanding of policy gradient approaches in real-world applications which tend to be partially observable.

==> Sections/11-SampleComplixity.tex <==
% \section{Sample Complexity Analysis}

==> Sections/3-1-Linear.tex <==
\subsection{Linear Quadratic}

Consider a episodic imperfect observation linear quadratic problem with the following hidden dynamical model:
\begin{align*}
    x_{t+1} = Ax_h + Ba_h+\omega_h
\end{align*}
and observation process of
\begin{align*}
    y_h = Cx_h + \nu_h
\end{align*}
which is observed after $x_h$ happens. Here $x\in\Re^n,y\in\Re^m, a\in \Re^d,A\in \Re^{n\times n},B\in \Re^{n\times d},C\in \Re^{m\times n}$. In LQs, we have $\omega_h$, and $\nu_h$ as mean zero random variables. The the cost function at each time step $h$ 
\begin{align*}
    \cost_h = \|y_h\|_Q^2+\|a_h\|_R^2
\end{align*}


where the $Q\in \Re^{n\times n},R\in \Re^{d\times d}$. Consider a episodic setting with episode length of $H$. 

Our goal is to minimize the total cost over space of linear control laws, i.e.

A bit of notation, $[H]=\lbrace 1,\ldots,H\rbrace$.


The expected cost of a given control law $K$ is as follows:
\begin{align*}
    \eta(K) = \E_K\left[\sum_{h=1}^{H}c_h\right]
\end{align*}

For simplicity of notation and analysis, we study the case where the only disturbance is the disturbance in the initial state distribution. In the case of known model we have:

This work seeks to characterize the behavior of (direct) policy
gradient methods, where  the policy is linearly parameterized, as
specified by a matrix $K \in
\Re^{d\times m}$ which generates the controls: $a_h = -K y_h$
for $h\in [H]$. 

We define the $S_h(K)$ as follows:
\begin{align*}
    S_h(K) = C^\top Q C+ C^\top K^\top R KC + (A-BKC)^\top S_{h+1}(K)  (A-BKC)
\end{align*}
resulting in 
\begin{align*}
    \eta(K) = \E_{x_0\sim P_0 }  \, x_1^\top S_1(K) x_1
\end{align*}

% we define $\Sigma_K = \E_{x_1\sim P_0 } \sum_{t=1}^H x_h x_h^\top$



\begin{lemma}\label{lem:gradexpression}
(Gradient in linear model) 
The gradient of the objective function is:
\begin{align*}
\nabla \eta(K) =2 \E\left[\sum_{h=1}^H \left( R K C+ B^\top S_2(K) (A-BKC)\right) x_h x_h^\top  C^\top\right] = 2\E\left[ \sum_{h=1}^H E_h(K) x_h x_h^\top  C^\top\right]
\end{align*}
where $E_h(K) = R K C+ B^\top S_h(K) (A-BKC)$
\end{lemma}



\begin{proof}
Observe:
\begin{align*}
V_K(x_1) =& x_1^\top S_1(K) x_1\\
=&x_1^\top\left(C^\top Q C+ C^\top K^\top R KC + (A-BKC)^\top S_{2}(K)  (A-BKC)\right)x_1\\
  =& x_1^\top\left(C^\top Q C+ C^\top K^\top R KC\right) x_1+
 x_1^\top (A-BKC)^\top S_{2}(K)  (A-BKC) x_1 \\
 =& x_1^\top\left(C^\top Q C+ C^\top K^\top R KC\right) x_1+ x_2^\top S_{2}(K)x_2
\end{align*}
Let $\nabla$ denote the gradient with respect to $K$, note that $\nabla C_K((A-BK)x_0)$ has two terms (one with respect to $K$ in the subscript and one with respect to the input $(A-BK)x_0$), this implies 
\begin{align*}
\nabla_K V_K(x_1)=& 2 R K C x_0 x_0^\top C^\top -2 B^\top S_2(K) (A-BKC) x_1 x_1^\top C^\top+  \nabla V_K(x_2)|_{x_2=(A-BKC)x_1}\\
=& 2 \sum_{h=1}^H \left( R K C+ B^\top S_2(K) (A-BKC)\right) x_h x_h^\top  C^\top
\end{align*}
using recursion and then expectations
completes the proof.
\end{proof}




==> Sections/4-Episodic.tex <==
We leave the analysis with respect to compatible function approximation to appendix~Subsection~\ref{sub:Compatible}.

In practice, depending on the problem at hand, either of the discussed approaches of computing the natural gradient might be applicable. Due to the close relationship between $\KL$ and Fisher information matrix Lemma~\ref{lem:KL-Fisher} and also the fact that the Fisher matrix is equal to second order Taylor expansion of $\KL$, instead of considering the area $\|\left(\theta-\theta'\right)^\top F\left(\theta-\theta'\right)\|_2\leq \delta$, or $\|\left(\theta-\theta'\right)^\top \nabla^2_{\theta'}\KL(\theta,\theta')|_{\theta'=\theta}\left(\theta-\theta'\right)\|_2\leq \delta$ for construction of the trust region, we can approximately consider $\KL(\theta,\theta')\leq \delta/2$. This relationship between these three approaches in constructing the trust region is used throughout this paper. %  Either of these approaches is application depends on the problem at hand %they result in sometimes different empirical performances and sometimes in different computation costs.
% It worth to note that, we show in the final result we do not need to compute the gigantic vector of $\phi(\tau;\theta)$ and $\omega$ for the exponentially many possible trajectories. 











==> macros.tex <==

\newcommand{\GTRPO}{\textsc{\small{GTRPO}}\xspace}
\newcommand{\GPPO}{\textsc{\small{GPPO}}\xspace}
\newcommand{\POMDP}{\textsc{\small{POMDP}}\xspace}
\newcommand{\MDP}{\textsc{\small{MDP}}\xspace}
\newcommand{\TRPO}{\textsc{\small{TRPO}}\xspace}
\newcommand{\PPO}{\textsc{\small{PPO}}\xspace}
\newcommand*{\Scale}[2][4]{\scalebox{#1}{$#2$}}
\newcommand{\cost}{c}
\newcommand{\vecy}{\vec y}
\newcommand{\history}{\mathfrak{H}}
\newcommand{\trans}{T}
\newcommand{\obs}{O}
\newcommand{\policy}{\Pi}
\newcommand{\vpi}{{\pi}}
\newcommand{\vobs}{\vec{o}}
\newcommand{\stait}{\omega}
\newcommand{\rxa}{\Gamma}
\newcommand{\rya}{\Upsilon}
\newcommand{\U}{\mathcal{U}}
\newcommand{\Est}{M_1}
\newcommand{\End}{M_2}
\newcommand{\Erd}{M_3}
\newcommand{\decompos}{\gamma}
\newcommand{\pertM}{\Delta M_3}
\newcommand{\pertMM}{\Delta \tilde{M_3}}
\newcommand{\samplenum}{m_s}
\newcommand{\reward}{\Psi}
\newcommand{\tuple}{\mathcal{M}}
\newcommand{\bellman}{\mathcal{E}}
\newcommand{\whole}{\tilde{\mathcal{M}}}
\newcommand{\approxim}{\breve{\mathcal{M}}}
\newcommand{\subst}{{\breve{\eta}}_{\vpi^*}}
\newcommand{\effect}{v}
\newcommand{\block}{\Xi}
\newcommand{\vect}{Vec}
\newcommand{\rprob}{z}
\newcommand{\past}{n}
\newcommand{\smucrl}{\textsc{\small{SM-UCRL}}\xspace}
\newcommand{\tslive}{\textsc{\small{TS-LIVE}}\xspace}
\newcommand{\olive}{\textsc{\small{OLIVE}}\xspace}
\newcommand{\cdp}{\textsc{{CDP}}\xspace}
\newcommand{\cdps}{\textsc{{CDPs}}\xspace}
\newcommand{\ts}{\textsc{TS}\xspace}
\newcommand{\ofu}{\textsc{OFU}\xspace}
\newcommand{\ucrl}{\textsc{\small{UCRL}}\xspace}
\newcommand{\mdp}{\textsc{\small{MDP}}\xspace}
\newcommand{\pomdp}{\textsc{\small{POMDP}}\xspace}
\newcommand{\Azuma}{\mathcal{J}}
\newcommand{\Dr}{D_{\text{ratio}}}
\newcommand{\Ke}{\mathcal{K}_\epsilon}
\newcommand{\Le}{L_\epsilon}
\newcommand{\w}{W}
\newcommand{\VV}{B}
\newcommand{\vv}{b}
\newcommand{\HH}{S}
\newcommand{\hhh}{s}
\newcommand{\deltaO}{d_O}

\newcommand*{\defeq}{\mathrel{\vcenter{\baselineskip0.5ex \lineskiplimit0pt
                     \hbox{\scriptsize.}\hbox{\scriptsize.}}}%
                     =}

% Misc symbols
\renewcommand{\Re}{\mathbb{R}}
\newcommand{\calP}{\mathcal P}
\newcommand{\PP}{\mathbb P}
\newcommand{\F}{\mathcal F}
\newcommand{\Z}{\mathcal Z}
\newcommand{\A}{\mathcal A}
\newcommand{\B}{\mathcal B}
\newcommand{\X}{\mathcal X}
\newcommand{\T}{\mathcal T}
\newcommand{\KL}{\mathcal D_{KL}}
\newcommand{\wKL}{\wh{\mathcal{D}}_{KL}}
\newcommand{\D}{\mathcal D}
\newcommand{\Gr}{\nabla_{\theta}}
\newcommand{\Greta}{\nabla \eta}
\newcommand{\Grrho}{\nabla \rho}
\newcommand{\Grphi}{\nabla_\phi}
\newcommand{\adv}{A}
\newcommand{\TN}{N}
\newcommand{\hh}{\hat h}
\newcommand{\hL}{\hat L}
\renewcommand{\L}{\mathcal L}
\newcommand{\Hyp}{\mathcal H}
\newcommand{\Y}{\mathcal Y}
\newcommand{\V}{\mathcal V}
\newcommand{\M}{\mathcal M}
\renewcommand{\S}{\mathcal S}
\newcommand{\C}{\mathcal C}
\newcommand{\K}{\mathcal K}
\newcommand{\E}{\mathbb E}
\newcommand{\calE}{\mathcal E}
\newcommand{\Cov}{\textnormal{Cov}}
%\newcommand{\V}{\mathbb V}
\newcommand{\Prob}{\mathbb P}
\newcommand{\I}{\mathbbm 1}
\newcommand{\N}{\mathcal N}
\newcommand{\balpha}{\boldsymbol \alpha}
\newcommand{\bmu}{\boldsymbol \mu}
\newcommand{\bSigma}{\boldsymbol \Sigma}
\newcommand{\bT}{\boldsymbol{T}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\MV}{\textnormal{MV}}
\newcommand{\hMV}{\widehat{\textnormal{MV}}}
\newcommand{\barmu}{\bar\mu}
\newcommand{\hmu}{\hat\mu}
\newcommand{\tmu}{\tilde\mu}
\newcommand{\barvar}{\bar\sigma^2}
%\newcommand{\hvar}{\hat\sigma^2}
\newcommand{\tvar}{\tilde\sigma^2}
\newcommand{\R}{\mathcal{R}}
\newcommand{\hR}{\widehat{\mathcal{R}}}
\newcommand{\tR}{\widetilde{\mathcal R}}
%\newcommand{\var}{\sigma^2}
\newcommand{\invdelta}{1/\delta}
\newcommand{\boldR}{\mathbb R}
\newcommand{\eps}{\varepsilon}
\newcommand{\mvlcb}{\textnormal{\texttt{MV-LCB }}}
\newcommand{\ucb}{\textnormal{\textsl{UCB }}}
\newcommand{\ucbv}{\textnormal{\textsl{UCB-V }}}
\newcommand{\mvlcbt}{\textnormal{\texttt{MV-LCB(t) }}}
\newcommand{\htheta}{\hat{\theta}}
\newcommand{\hi}{\hat{i}}
\newcommand{\btheta}{\bar{\theta}}
\newcommand{\tTheta}{\widetilde{\Theta}}

\newcommand{\cvar}{\textnormal{C}}
\newcommand{\hcvar}{\widehat{\textnormal{C}}}
\newcommand{\var}{\textnormal{V}}
\newcommand{\hvar}{\widehat{\textnormal{V}}}
\newcommand{\Pinit}{P_\varnothing}



\newcommand{\avg}[2]{\frac{1}{#2} \sum_{#1=1}^{#2}}
\newcommand{\hDelta}{\widehat{\Delta}}
\newcommand{\hGamma}{\widehat{\Gamma}}

\newcommand{\wt}{\widetilde}
\newcommand{\wh}{\widehat}
\newcommand{\wb}{\overline}
 \newcommand{\mbb}{\mathbbm}

% Propositions
%
%\newtheoremstyle{dotless}{}{}{\itshape}{}{\bfseries}{}{ }{}
%\theoremstyle{dotless}
% \newtheorem{lemma}{Lemma}
\newtheorem{assumption}{Assumption}

% \newtheorem{definition}{Definition}
% \newtheorem{theorem*}{Theorem}
% \newtheorem{corollary}{Corollary}
% \newtheorem{proposition}{Proposition}
%\newtheorem{definition}{Definition}
% \newtheorem{theorem}{Theorem}
% \newtheorem{definition}{Definition}
% \newtheorem{remark}{Remark}
% \newtheorem{proof}{Proof}
% \newtheorem*{proof*}{Proof}
% Misc
%\newcommand{\note}[1]{\textbf{Note.} \textit{#1}}
%\newcommand{\TODO}[1]{(\textbf{TODO: {#1}})}
%\renewcommand{\remark}[1]{\textbf{Remark #1.}}





\newcommand*{\eg}{e.g.\@\xspace}
\newcommand*{\eq}{Eq.~}
\newcommand*{\fig}{Fig.~}
\newcommand*{\lem}{Lem.~}
\newcommand*{\tab}{Tab.~}
\newcommand*{\appx}{Apx.~}
\newcommand*{\sect}{Sec.~}
\newcommand*{\thm}{Thm.~}
\newcommand*{\alg}{Alg.~}
\newcommand*{\prop}{Prop.~}
